Parameter-free Regret in High Probability with Heavy Tails

We present new algorithms for online convex optimization over unbounded domains that obtain parameter-free regret in high-probability given access only to potentially heavy-tailed subgradient estimates. Previous work in unbounded domains considers only in-expectation results for sub-exponential subgradients. Unlike in the bounded domain case, we cannot rely on straight-forward martingale concentration due to exponentially large iterates produced by the algorithm. We develop new regularization techniques to overcome these problems. Overall, with probability at most $\delta$, for all comparators $\mathbf{u}$ our algorithm achieves regret $\tilde{O}(\| \mathbf{u} \| T^{1/\mathfrak{p}} \log (1/\delta))$ for subgradients with bounded $\mathfrak{p}^{th}$ moments for some $\mathfrak{p} \in (1, 2]$.

==> fixed_notes.tex <==

\section*{Fixed}
\begin{enumerate}
    \item use Lemma \ref{lemma:scaled_sum_berinstein} for MDS $\{X_t, \mathcal{F}_t \}$ when $X_t$ is $(\sigma, b)$ subexponential. $\sigma, b$ are fixed quantity here.
    \item Fixed appendix \ref{sec:app_bernstein}, now theorem \ref{thm:main_sub_exp} has the right constant with new concentration bound. Replaced all $\ln$, now $\log$ denote the natural logarithmic.
    \item Fixed appendix \ref{sec:app_clipping}, use lemma \ref{lemma:truncated_grad_concentration} for a tail bound for $\sum_{t=1}^{T} \hat{g}_t^2$. Since $\E[\hat{g}_t^2 \| w_t] \leq \sigma^2$ and $|\hat{g}_t| \leq \tau$. $\sigma$ and $\tau$ are both fixed quantity.
    \item I really think appendix are done... 
    \item the density $\pi(\eta)$ in the proof for theorem \ref{thm:mdsconcentration} is a bit wired... I don't see why there is an argument of $x$. and equation (12) is not quite true when taking derivative with equation (11) 
    \item theorem \ref{thm:main_heavy}, maybe keep one results in the main text, they don't look much different with $\tidel{O}(\cdot)$. 
    \item Theorem \ref{thm:heavy_nd} also identical. A bit confused about what to keep in $\tilde{O}(\cdot)$. I just check each variable, take their highest order and ignore anything below $\log(\cdot)$.
    \item capitalised Theorem, Lemma, Proposition. equation ()
    
\end{enumerate}
